RoboColosseum: Evaluating Physical Intelligence at Scale In-The-Wild

General-purpose robot policies must work across robots, tasks, and environments, yet the variation that makes physical trials informative also makes them difficult to reproduce. We introduce RoboColosseum, a distributed evaluation framework that combines unified policy serving and standardized protocols across a network of locally operated robots in diverse environments. Our initial study evaluates five vision-language-action (VLA) policies and three frontier AI agents across four embodiments (SO-101, Franka, Bimanual-YAM, and G1 Humanoid). The Open Track compares models without task-specific adaptation in blinded, pairwise trials under matched local conditions. The Fine-tune Track measures how well VLA policies adapt to 20 tasks across all four embodiments when each policy receives the same 100 demonstrations per task. Across 5,699 pairwise Open Track comparisons at 124 sites, frontier agents rival specialized VLA policies, while all systems struggle to complete open-world tasks reliably. After fine-tuning, GR00T N1.7 leads on SO-101 and pi0.5 leads on Franka and Bimanual-YAM. Policy rankings show weak agreement across embodiment-specific task suites (Kendall W = 0.24). Open Track rankings poorly predict relative performance after fine-tuning, with substantial rank reversals on all three embodiments shared between tracks. Measuring partial progress reveals differences that task success alone misses. On the G1 Humanoid, no policy completes any of the five tasks, yet average progress ranges from 13.3% to 23.2% across policies. Open Track rankings stabilize as trials accumulate, and active matchmaking achieves comparable ranking agreement with substantially fewer physical trials than uniform sampling. These results show how distributed physical evaluation can reveal where robot policies generalize, how well they adapt to new tasks, and how far they progress on tasks they fail to complete.

==> tables/fig_embodiment_coverage.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results/performance_consistency/embodiment_coverage_absolute.png}
    \caption{\textbf{Performance under increasing embodiment coverage.}
    Worst-case Fine-tuning Track progress score (PS) as increasingly larger sets of robot embodiments are considered. For each set, the model's lowest embodiment-level PS defines its performance floor; values are averaged over all embodiment subsets of the same size. Higher values indicate more consistent performance across embodiments.}
    \label{fig:embodiment_coverage}
\end{figure}


==> tables/fig_finetuning_embodiment_summary.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{images/results/task_adaptation/finetuning_embodiment_summary_ci.png}
    \caption{\textbf{Fine-tuning performance across embodiments.} Embodiment-level (a) normalized progress score (PS) and (b) success rate (SR) for the five evaluated VLA policies. Each point is the equal-weight mean over the five tasks for that embodiment, with error bars showing 95\% bootstrap confidence intervals. Higher values indicate better performance. $\dagger$ denotes an embodiment-level result that includes a task whose evaluation was stopped early for safety.}
    \label{fig:finetuning_embodiment_summary}
\end{figure}


==> tables/fig_open_track_elo.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{images/open_track_elo_ci.pdf}
    \caption{\textbf{Open track placeholder.} }
    \label{fig:open_track_elo}
\end{figure}


==> tables/fig_ranking_convergence.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results/ranking_reliability/ranking_convergence_random_only.png}
    \caption{\textbf{Open Track ranking convergence with evaluation budget.}
    Agreement between the BTD ranking estimated from randomly subsampled Open Track comparisons and the ranking obtained from the full dataset. The x-axis gives the number of physical pairwise comparisons and the y-axis gives pairwise ordering agreement with the full-data ranking. The solid line shows the mean across repeated random subsamples and the shaded region shows the 95\% interval across subsamples. Horizontal dashed lines mark 90\% and 95\% ranking agreement.}
    \label{fig:ranking_convergence}
\end{figure}


==> tables/fig_ranking_convergence_dcr.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/results/scaling_effect/evaluation_scale_dcr.png}
\caption{\textbf{Effect of evaluation scale on Open Track ranking stability.}
At each evaluation budget, we sample 200 random subsets containing all eight systems, fit DCR using only those evaluations, and compare the resulting ranking with the DCR ranking obtained from the full 5,699-evaluation dataset. The line shows the mean agreement across the 200 subsets, and the shaded region spans the 2.5th--97.5th percentiles. Dashed lines mark 90\% and 95\% mean ranking agreement.}
    \label{fig:evaluation_scale_dcr}
\end{figure}


==> tables/fig_ranking_method_robustness.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/results/ranking_reliability/ranking_method_robustness_by_embodiment.png}
    \caption{\textbf{Open Track ranking robustness across ranking formulations.}
    Model rankings under DCR, BTD, sequential Elo, and average pairwise score for (a) SO-101, (b) DROID/Franka, and (c) Bimanual-YAM. Each line tracks the rank of one model across the four formulations, with rank 1 denoting the highest-ranked model. Only systems evaluated on the corresponding embodiment are included. Above each panel, $\rho$ reports Spearman's rank correlation between each alternative ranking and DCR.}
    \label{fig:ranking_method_robustness}
\end{figure}


==> tables/fig_rq2_task_relative_success.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/results/task_adaptation/rq2_task_relative_success.pdf}
    \caption{\textbf{Task-specific performance after fine-tuning.}
    Each cell shows a policy's success rate relative to the mean success rate of the five policies on the same task, in percentage points; blue indicates above-average and red below-average performance. The bottom row shows the task mean success rate, while the right column counts the tasks on which each policy achieves the highest success rate. Unitree G1 tasks are hatched because no policy achieves full-task success.}
    \label{fig:rq2_task_relative_success}
\end{figure}


==> tables/fig_site_split_reliability.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/results/ranking_reliability/site_split_ranking_reliability.png}
\caption{\textbf{Consistency of DCR rankings across independent evaluation-site subsets.}
For each embodiment, evaluation sites are repeatedly divided into two disjoint subsets, and DCR is fit independently on each half. Points show the mean fraction of model pairs whose relative ordering agrees between the two rankings, and error bars show the 2.5th--97.5th percentile across valid random splits. The annotated $\rho$ is the mean Spearman rank correlation between the two rankings. Higher values indicate that the leaderboard is less sensitive to which subset of evaluation sites contributes the data.}
    \label{fig:site_split_reliability}
\end{figure}


==> tables/open_track_leaderboard_balanced.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Embodiment-balanced Open Track leaderboard.} Panel A compares the five VLA policies across all three shared Open Track embodiments (SO101, DROID, YAM); Panel B compares all eight systems on the two embodiments shared by all models with at least 20 comparisons each (SO101, YAM); DROID is left out because gpt-6-astra has only 18 comparisons there. On each embodiment, a Bradley--Terry--Davidson model is fitted separately to the comparisons among the panel's models; $Q_{m,e}$ is the expected pairwise score (win $=1$, tie $=\tfrac{1}{2}$) of model $m$ against an average model of that fit, so 50\% equals the panel average. The balanced score $Q_m$ is the unweighted mean of $Q_{m,e}$ over the panel's embodiments: embodiments are weighted equally rather than according to their number of evaluations. 95\% intervals: 1000 stratified bootstrap resamples (comparisons resampled within each embodiment and every embodiment refitted). $N$: comparisons of the model used in the panel. Best and second-best values within each panel are marked in \textbf{bold} and \underline{underline}; a dash marks an embodiment not used in that panel.}
\label{tab:open_track_leaderboard_balanced}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}clcccccr@{}}
\toprule
\multirow{2}{*}{\textcolor{RTBlue}{\textbf{Rank}}} & \multirow{2}{*}{\textcolor{RTBlue}{\textbf{Model}}} & \multirow{2}{*}{\textcolor{RTBlue}{\textbf{Balanced $Q_m$}}} & \multirow{2}{*}{\textcolor{RTBlue}{\textbf{95\% CI}}} & \multicolumn{3}{c}{\textcolor{RTBlue}{\textbf{Per-embodiment $Q_{m,e}$}}} & \multirow{2}{*}{\textcolor{RTBlue}{\textbf{$N$}}} \\
\cmidrule(lr){5-7}
 & & & & \textcolor{RTBlue}{\textbf{SO101}} & \textcolor{RTBlue}{\textbf{DROID}} & \textcolor{RTBlue}{\textbf{YAM}} & \\
\midrule
\multicolumn{8}{@{}l}{\textcolor{RTBlue}{\textbf{Panel A: 5 VLA policies, SO101 + DROID + YAM}}} \\
1 & MolmoAct2 & \rtbest{58.0} & [55.4, 60.9] & \rtsecond{54.1} & \rtbest{69.7} & \rtsecond{50.3} & 1877 \\
2 & LingBot-VLA v2 & \rtsecond{56.5} & [54.1, 59.0] & 53.1 & 43.6 & \rtbest{72.6} & 1716 \\
3 & G0.5 & 48.2 & [45.6, 50.5] & 37.4 & \rtsecond{64.1} & 43.0 & 1732 \\
4 & $\pi_{0.5}$ & 44.6 & [41.6, 47.4] & \rtbest{63.9} & 28.8 & 41.2 & 1237 \\
5 & GR00T N1.7 & 42.1 & [39.5, 44.7] & 41.5 & 43.7 & 41.2 & 1890 \\
\midrule
\multicolumn{8}{@{}l}{\textcolor{RTBlue}{\textbf{Panel B: 8 systems, SO101 + YAM}}} \\
1 & claude-opus-5-5 & \rtbest{63.4} & [58.3, 68.6] & \rtsecond{70.3} & \textemdash & \rtsecond{56.4} & 183 \\
2 & gpt-6-astra & \rtsecond{60.8} & [56.4, 64.9] & \rtbest{72.2} & \textemdash & 49.4 & 329 \\
3 & LingBot-VLA v2 & 57.8 & [53.9, 61.7] & 45.5 & \textemdash & \rtbest{70.1} & 704 \\
4 & grok-4.7 & 53.1 & [48.3, 57.4] & 50.4 & \textemdash & 55.8 & 343 \\
5 & MolmoAct2 & 47.4 & [43.8, 51.3] & 46.0 & \textemdash & 48.9 & 702 \\
6 & $\pi_{0.5}$ & 46.0 & [42.0, 49.9] & 52.7 & \textemdash & 39.3 & 688 \\
7 & GR00T N1.7 & 35.7 & [32.2, 39.2] & 32.7 & \textemdash & 38.7 & 692 \\
8 & G0.5 & 34.9 & [31.7, 37.9] & 29.2 & \textemdash & 40.6 & 697 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ranking_method_comparison.tex <==
\begin{table}[t]
\centering
\small
\caption{Open Track ranking under three aggregation methods (Elo: chronological order, $K=32$, initial 1000, scale 400).}
\label{tab:ranking_methods}
\begin{tabular}{lcccccc}
\toprule
Model & Pairwise score (\%) & Rank & Elo & Rank & BTD $\theta$ & Rank \\
\midrule
claude-opus-5-5 & 59.3 & 2 & 1055.3 & 3 & $+0.54$ & 1 \\
MolmoAct2 & 63.8 & 1 & 1002.8 & 5 & $+0.44$ & 2 \\
gpt-6-astra & 53.6 & 3 & 1080.1 & 1 & $+0.33$ & 3 \\
grok-4.7 & 51.2 & 5 & 921.0 & 7 & $+0.25$ & 4 \\
G0.5 & 53.5 & 4 & 1003.2 & 4 & $+0.03$ & 5 \\
LingBot-VLA v2 & 51.1 & 6 & 1067.8 & 2 & $-0.07$ & 6 \\
GR00T N1.7 & 40.5 & 7 & 960.3 & 6 & $-0.60$ & 7 \\
$\pi_{0.5}$ & 34.3 & 8 & 909.5 & 8 & $-0.92$ & 8 \\
\bottomrule
\end{tabular}
\par\vspace{2pt}
\parbox{\linewidth}{\footnotesize Rank correlations: Pairwise score vs Elo: Spearman 0.50, Kendall 0.36; Pairwise score vs BTD: Spearman 0.95, Kendall 0.86; Elo vs BTD: Spearman 0.48, Kendall 0.36}
\end{table}


==> tables/rq1_agent_vla_vs_difficulty.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/results/openworld_capabilities/rq1_agent_vla_vs_difficulty.png}
    \caption{\textbf{Relative and absolute Agent - VLA performance across task difficulty.}
    We consider matched Open Track evaluations in which a general-purpose agent and a VLA policy are evaluated on the same task and local setup. (a) Agent comparison score, computed as $(\text{agent wins}+0.5\times\text{ties})/N$; 50\% indicates parity, while values above 50\% favor agents. (b) Full-task success rate on the same matched evaluations. Error bars show 95\% intervals, and the counts below each panel report the number of matched evaluations and their outcomes.}
    \label{fig:agent_vla_vs_difficulty}
\end{figure}

